Beyond Gemini-3-Pro: Revisiting LLM Routing and Aggregation at Scale

Large Language Models (LLMs) have rapidly advanced, with Gemini-3-Pro setting a new performance milestone. In this work, we explore collective intelligence as an alternative to monolithic scaling, and demonstrate that open-source LLMs' collaboration can surpass Gemini-3-Pro. We first revisit LLM routing and aggregation at scale and identify three key bottlenecks: (1) current train-free routers are limited by a query-based paradigm focusing solely on textual similarity; (2) recent aggregation methods remain largely static, failing to select appropriate aggregators for different tasks;(3) the complementarity of routing and aggregation remains underutilized. To address these problems, we introduce JiSi, a novel framework designed to release the full potential of LLMs' collaboration through three innovations: (1) Query-Response Mixed Routing capturing both semantic information and problem difficulty; (2) Support-Set-based Aggregator Selection jointly evaluating the aggregation and domain capacity of aggregators; (3) Adaptive Routing-Aggregation Switch dynamically leveraging the advantages of routing and aggregation. Comprehensive experiments on nine benchmarks demonstrate that JiSi can surpass Gemini-3-Pro with only 47% costs by orchestrating ten open-source LLMs, while outperforming mainstream baselines. It suggests that collective intelligence represents a novel path towards Artificial General Intelligence (AGI).

==> alg/method.tex <==
\begin{algorithm*}[htbp]
\caption{JISI inference. Vector operations in PyTorch~\cite{paszke2019pytorchimperativestylehighperformance} style}
\label{alg:stpp}
\KwIn{New question $x$ for inferece; LLMs $\left\{\boldsymbol{A}_1,\dots,\boldsymbol{A}_M\right\}$; Embedder $\boldsymbol{f}_1$; Prebuilt embedding bank containing $\boldsymbol{e}\in\mathbb{R}^{N\times{d}},\,\boldsymbol{r}\in\mathbb{R}^{M\times{N}\times{d}},\,\boldsymbol{v}\in\mathbb{R}^{N\times{M}},\,\boldsymbol{c}\in\mathbb{R}^{M\times{N}\times1}$; Hyperparameters $K,\,N^{base},\,\beta,\,\gamma,\,\epsilon,\,\sigma,\,\delta,\,t$;}
\KwOut{Response $\hat{y}$ \wrt $x$;}
\tcp{Dynamic Aggregator Selection}
$\rhd$ $sim\leftarrow\boldsymbol{e}.\operatorname{matmul}\left(\boldsymbol{f}_1\left(x\right)\right)$;\quad\tcp{$sim\in\mathbb{R}^{N\times1}$}
$\rhd$ $q\_mask\leftarrow\left(sim\ge\left(\gamma*sim.\operatorname{topk}\left(\operatorname{k}=N^{base}\right).\operatorname{values}\left[-1\right]\right)\right)$;\\
$\rhd$ $score\leftarrow\left(\boldsymbol{v}*sim*q\_mask\right).\operatorname{sum}\left(\operatorname{dim}=0\right)$;\quad\tcp{$score\in\mathbb{R}^{M}$}
$\rhd$ $\left(m\_mask,\,agg\right)\leftarrow\left(\left(score\ge{s}core.\operatorname{topk}\left(\operatorname{k}=K\right).\operatorname{values}\left[-1\right]\right),\,score.\operatorname{argmax}\left(\right)\right)$;\\
\tcp{Response-based Reroute}
\For{$i\ \boldsymbol{\operatorname{in}}\ \operatorname{torch}.\operatorname{arange}\left(M\right)\left[m\_mask\right]$}{
$\rhd$ $res\leftarrow\boldsymbol{A}_{i+1}\left(x\right)$;\quad\tcp{$cost$ collected}
$\rhd$ $r\_sim\left[i\right]\leftarrow\boldsymbol{r}\left[i\right].\operatorname{matmul}\left(\boldsymbol{f}_1\left(res\right)\right)$;\quad\tcp{$r\_sim\in\mathbb{R}^{M\times{N}\times1}$}
$\rhd$ $c\_sim\left[i\right]\leftarrow\left(\boldsymbol{c}\left[i\right]^2-cost^2\right).\operatorname{abs}\left(\right)$;\quad\tcp{$c\_sim\in\mathbb{R}^{M\times{N}\times1}$}
$\rhd$ $c\_sim\left[i\right]\leftarrow\left(1-c\_sim[i].\operatorname{div}\left(\left(c\_sim\left[i\right]*q\_mask\right).\operatorname{max}\left(\right)\right)\right)$;\\}
$\rhd$ $\left(r\_sim,\,c\_sim\right)\leftarrow\left(r\_sim.\operatorname{sum}\left(\operatorname{dim}=0\right),\,c\_sim.\operatorname{sum}\left(\operatorname{dim}=0\right)\right)$;\\
$\rhd$ $sim\leftarrow\left(\left(\epsilon{K}*q\_sim+\sigma*r\_sim+\delta*c\_sim\right)*q\_mask\right)$;\\
$\rhd$ $q\_mask\leftarrow\left(sim\ge\left(sim.\operatorname{topk}\left(\operatorname{k}=\left(\beta*q\_mask.\operatorname{sum}\left(\right)\right).\operatorname{long}\left(\right)\right).\operatorname{values}\left[-1\right]\right)\right)$;\\
$\rhd$ $score\leftarrow\left(\boldsymbol{v}*sim*q\_mask\right).\operatorname{sum}\left(\operatorname{dim}=0\right)$;\\
\tcp{Adaptive Aggregation}
$\rhd$ $m\_mask\leftarrow\left(\left(score\ge{s}core.\operatorname{topk}\left(\operatorname{k}=K\right).\operatorname{values}\left[-1\right]\right)*\left(score.\operatorname{div}\left(score.\operatorname{max}\left(\right)\right)\ge{t}\right)\right)$;\\
\eIf{$\left(m\_mask.\operatorname{sum}\left(\right)=1\right)$}{
$\rhd$ $\hat{y}\leftarrow\boldsymbol{A}_{score.\operatorname{argmax}\left(\right)}\left(x\right)$;\\}{
$\rhd$ $\hat{y}\leftarrow\boldsymbol{A}_{agg}\left(\operatorname{sum}\left(\boldsymbol{A}_i\left(x\right)\ \boldsymbol{\operatorname{for}}\ i\ \boldsymbol{\operatorname{in}}\ \operatorname{torch}.\operatorname{arange}\left(M\right)\left[m\_mask\right]\right)\right)$;}
\end{algorithm*}

